Study of Io's sodium jets with the TRAPPIST telescopes

Io is the most volcanically active body in the Solar System. This volcanic activity results in the ejection of material into Io's atmosphere, which may then escape from the atmosphere to form various structures in the jovian magnetosphere, including the plasma torus and clouds of neutral particles. The physical processes involved in the escape of particles - for example, how the volcanoes of Io provide material to the plasma torus - are not yet fully understood. In particular, it is not clear to what extent the sodium jet, one of the sodium neutral clouds related to Io, is a proxy of processes that populate the various reservoirs of plasma in Jupiter's magnetosphere. Here, we report on observations carried out over 17 nights in 2014-2015, 30 nights in 2021, and 23 nights in 2022-2023 with the TRAPPIST telescopes, in which particular attention was paid to the sodium jet and the quantification of their physical properties (length, brightness). It was found that these properties can vary greatly from one jet to another and independently of the position of Io in its orbit. No clear link was found between the presence of jets and global brightening of the plasma torus and extended sodium nebula, indicating that jets do not contribute straightforwardly to their population. This work also demonstrates the advantage of regular and long-term monitoring to understanding the variability of the sodium jet and presents a large corpus of jet detections against which work in related fields may compare.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
